Meta-Curvature

We propose meta-curvature (MC), a framework to learn curvature information for better generalization and fast model adaptation. MC expands on the model-agnostic meta-learner (MAML) by learning to transform the gradients in the inner optimization such that the transformed gradients achieve better generalization performance to a new task. For training large scale neural networks, we decompose the curvature matrix into smaller matrices in a novel scheme where we capture the dependencies of the model's parameters with a series of tensor products. We demonstrate the effects of our proposed method on several few-shot learning tasks and datasets. Without any task specific techniques and architectures, the proposed method achieves substantial improvement upon previous MAML variants and outperforms the recent state-of-the-art methods. Furthermore, we observe faster convergence rates of the meta-training process. Finally, we present an analysis that explains better generalization performance with the meta-trained curvature.

==> temp.tex <==
\begin{table}[t]
\caption{The results on miniImagenet and tieredImagenet (5-way classification) with WRN-28-10. $^\ddagger$ indicates that both meta-train and meta-validation are used during meta-training. $^\mathsection$ indicates that 15-shot training was adopted for meta-training and 1 or 5 shot was used for testing.}
\vskip -0.1in
\label{table:miniimagenet_wrn}
\begin{center}
\begin{small}
\begin{tabular}{lccccc}
\toprule
& &\multicolumn{2}{c}{miniImagenet} & \multicolumn{2}{c}{tieredImagenet} \\
\midrule
& Backbone & 1-shot & 5-shot & 1-shot & 5-shot \\
\midrule
TADAM \cite{Oreshkin-nips18}& ResNet-12 & 58.50 $\pm$ 0.30 & 76.70 $\pm$ 0.30 & $\cdot$ & $\cdot$\\
MetaOptNet$^\mathsection$ \cite{metaopt}& ResNet-12 & 62.64 $\pm$ 0.61 & 78.63 $\pm$ 0.46 & 65.99 $\pm$ 0.72 & 81.56 $\pm$ 0.53 \\
MetaOptNet$^\ddagger$ $^\mathsection$ \cite{metaopt}& ResNet-12 & \textbf{64.09} $\pm$ \textbf{0.62} & \textbf{80.00} $\pm$ \textbf{0.45} & 65.81 $\pm$ 0.74 & \textbf{81.75} $\pm$ \textbf{0.53} \\
\midrule
\cite{Qiao-cvpr18}$^\ddagger$ & WRN-28-10 & 59.60 $\pm$ 0.41 & 73.74 $\pm$ 0.19 & $\cdot$ & $\cdot$ \\
LEO$^\ddagger$ \cite{rusu-iclr19}& WRN-28-10 & 61.76 $\pm$ 0.08 & 77.59 $\pm$ 0.12 & 66.33 $\pm$ 0.05 & 81.44 $\pm$ 0.09 \\
\midrule
Meta-SGD   &   WRN-28-10  & 56.58 $\pm$ 0.21 &  68.84 $\pm$ 0.19 & 59.75 $\pm$ 0.25 & 69.04 $\pm$ 0.22 \\
%MC1        &   WRN-28-10  & 59.70 $\pm$ 0.22 &  $\pm$ & 63.02 $\pm$ 0.25 & 75.44 $\pm$ 0.21 \\
MC2        &   WRN-28-10  & 58.80 $\pm$ 0.21 &  74.49 $\pm$ 0.16 & 65.54 $\pm$ 0.24 & 78.98 $\pm$ 0.19 \\
MC2$^\ddagger$ & WRN-28-10  &  60.93 $\pm$ 0.22 &  74.45 $\pm$ 0.17 & \textbf{66.76} $\pm$ \textbf{0.24} & 79.83 $\pm$ 0.18  \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.3in
\end{table}
